Rethinking Missing Data: Aleatoric Uncertainty-Aware Recommendation

Historical interactions are the default choice for recommender model training, which typically exhibit high sparsity, i.e., most user-item pairs are unobserved missing data. A standard choice is treating the missing data as negative training samples and estimating interaction likelihood between user-item pairs along with the observed interactions. In this way, some potential interactions are inevitably mislabeled during training, which will hurt the model fidelity, hindering the model to recall the mislabeled items, especially the long-tail ones. In this work, we investigate the mislabeling issue from a new perspective of aleatoric uncertainty, which describes the inherent randomness of missing data. The randomness pushes us to go beyond merely the interaction likelihood and embrace aleatoric uncertainty modeling. Towards this end, we propose a new Aleatoric Uncertainty-aware Recommendation (AUR) framework that consists of a new uncertainty estimator along with a normal recommender model. According to the theory of aleatoric uncertainty, we derive a new recommendation objective to learn the estimator. As the chance of mislabeling reflects the potential of a pair, AUR makes recommendations according to the uncertainty, which is demonstrated to improve the recommendation performance of less popular items without sacrificing the overall performance. We instantiate AUR on three representative recommender models: Matrix Factorization (MF), LightGCN, and VAE from mainstream model architectures. Extensive results on two real-world datasets validate the effectiveness of AUR w.r.t. better recommendation results, especially on long-tail items.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> method.tex <==
\section{METHOD}\label{sec:method}

% We first introduce the definition of our aleatoric uncertainty in recommendation systems in Section \ref{sec:method-overall}. %as well as an user-batch training strategy 
% In Section \ref{unestimator}, we present how to properly estimate the uncertainty.
% The specific training procedures for both the backbone expectation estimator and uncertainty estimator are provided in Section \ref{sec:training}. 
% In Section \ref{sec:algo}, we show theoretical and empirical evidence to support our method.
% Finally, we discuss and compare the heuristic re-weight methods with our method in Section \ref{sec:discussion}.
% \begin{algorithm}[!h]
%     \caption{algorithm of SUM}
%     \label{alg:AOA}
%     \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%     \renewcommand{\algorithmicensure}{\textbf{Output:}}
%     \begin{algorithmic}[1]
%         \REQUIRE $A$, $B$, $C$  %%input
%         \ENSURE EEEEE    %%output
        
%         \STATE  AAAAA
%         \WHILE{$A=B$}
%             \STATE BBBBB
%         \ENDWHILE
        
%         \FOR{each $i \in [1,10]$}
%             \IF {$C = 0$}
%                 \STATE CCCCC
%             \ELSE
%                 \STATE DDDDD
%             \ENDIF
%         \ENDFOR
        
%         \RETURN EEEEE
%     \end{algorithmic}
% \end{algorithm}
% \begin{algorithm}[h]
%   \SetAlgoLined
%   \KwData{Hyperparameters $K$,$\alpha$,$\beta$,$\gamma$,$\lambda$,$\mu$}
%   \KwResult{Fixed prediction $Pred_{ui}$ for each (u,i) }
%   initialization $\theta$, $\Phi$\;
%   \textbf{Backbone Training Process}\;
%   \While{not converge }{
%   for each (u,i) $r_{ui}=f_{\theta}(u,i)$\;
%   Update parameter $\theta$ by Equation \ref{loss_backbone}\;
%   }
%   \textbf{Uncertainty Estimator Training Process}\;
%   \while{not converge}{
%   for each (u,i) $r_{ui}=f_{\theta}(u,i)$\;
%   for each (u,i) $s_{ui}=h_{\phi}(u,i)$\;
%   Update parameter $\phi$ by Equation \ref{loss}\;
%   }
%   Fix the original model prediction by aleatoric uncertainty $Pred_{ui}=\lambda r_{ui} + (1-\lambda)\sqrt{ \frac{e^{s_{ui}}}{K}}$
  
  
  
%   \caption{Overall Training Process for AUR}
%   \label{train_process}
% \end{algorithm}
\textbf{Problem Formulation. }%\label{sec:problem}
Suppose we have an implicit %recommendation
feedback dataset 
$\mathcal{D}$ with $m$ users and $n$ items. The set of users and items are represented as $\mathcal{U}$ and $\mathcal{I}$. 
%For any $u \in \mathcal{U}$ and $i \in \mathcal{I}$, the label of pair $(u,i)$ can be represented as:
% Under All Missing Are Negative assumption, the implicit data can be formulated as:
% \begin{equation}
%     Y_{ui}=
%   \begin{cases}
%   1 &\mbox{if $u$ has consumed $i$,}\\
%   0 &\mbox{else.}
%   \end{cases}
%   \label{label}
%   \end{equation}
For any $u \in \mathcal{U}$ and $i \in \mathcal{I}$, the label of pair $(u,i)$ is $Y_{ui}=1$, if $u$ has consumed $i$, and $Y_{ui}=0$ otherwise.
% \begin{equation}
%     Y_{ui}=
%   \begin{cases}
%   1 &\mbox{if $u$ has consumed $i$,}\\
%   0 &\mbox{else.}
%   \end{cases}
%   \label{label}
%   \end{equation}
% Assume that we have a backbone recommendation model trained as maximuming likelihood of Normal Distribution$f_{\theta}$. The prediction matrix is defined as $R={r_{ui}}_{m \times n}$. W
Let $\mathcal{R}=\{ r_{ui} \}_{m \times n}$ denote the predictions given by a %well-trained
backbone model (\eg MF) parameterized with $\theta$, \ie we have $r_{ui}=f_{\theta}(u,i)$. 
We design a two-stage optimization strategy. In the backbone training stage, we update the parameter $\theta$ of the backbone model.
%, where $r_{ui}$ is parameterized with a neural network denoted as $r_{ui}=f_{\theta}(u,i)$.
We assume that $Y_{ui} \sim N(r_{ui},\sigma_{ui}^2)$ and treat the $\sigma_{ui}^2$ as aleatoric uncertainty. We design a light uncertainty estimator to obtain the aleatoric uncertainty as $\sigma_{ui}^2=g_{\phi}(u,i)$, which can effieciently serve online. In the uncertainty estimator training stage, we update the parameter $\phi$ to the uncertainty estimator. After two-stage training, we linear combine the $r_{ui}$ and $\sigma_{ui}$ to recommend items.
% We assume that $Y_{ui} \sim N(r_{ui},\sigma_{ui}^2)$ and learn the variance $\sigma_{ui}^2$ as our aleatoric uncertainty. 
%The backbone model with a neural network parameterized by $\theta$ is denoted as $r_{ui}=f_{\theta}(u,i)$.
%The sets of backbone model and uncertainty estimators are $\theta$ and $\phi$ respectively. 
% The backbone prediction and uncertainty estimation can be represented as $r_{ui}=f_{\theta}(u,i)$ and $\sigma_{ui}^2=g_{\phi}(u,i)$, where $g_{\phi}(\cdot, \cdot)$ denotes the uncertainty estimator parameterized with $\phi$. 
% The overall training process is organized as Algorithm \ref{train_process}.
% Finally, we learn the uncertainty by our AUR framework and directly recommend items according to the aleatoric uncertainty. 
% 
%We evaluate our method on the holdout dataset in the testing stage. 

%For a more comprehensive evaluation of our model, we adopt three different evaluation protocols, which are named as \textbf{Overall Evaluation}, \textbf{Tail Absolute Evaluation}, and \textbf{Tail Relative Evaluation} (see Section~\ref{ssec:exp_setting} for details).


%In this section, 
%In the following, we first introduce the definition of aleatoric uncertainty in recommendation, and present how to properly estimate the uncertainty. We then describe training procedures for the backbone expectation estimator and uncertainty estimator, followed by some analysis.
%. Finally, we provide some analysis and discussion of our approach.

% \begin{algorithm}[h]
%   \SetAlgoLined
%   \KwData{Hyperparameters $K$,$\alpha$,$\beta$,$\gamma$,$\lambda$,$\mu$}
%   \KwResult{Fixed prediction $Pred_{ui}$ for each (u,i) }
%   initialization $\theta$, $\Phi$\;
%   \textbf{Backbone Training Process}\;
%   \While{not converge }{
%   for each (u,i) $r_{ui}=f_{\theta}(u,i)$\;
%   Update parameter $\theta$ by Equation \ref{loss_backbone}\;
%   }
%   \textbf{Uncertainty Estimator Training Process}\;
%   \While{not converge }{
%   for each (u,i) $r_{ui}=f_{\theta}(u,i)$\;
%   for each (u,i) $s_{ui}=h_{\phi}(u,i)$\;
%   Update parameter $\phi$ by Equation \ref{loss}\;
%   }
%   Fix the original model prediction by aleatoric uncertainty $Pred_{ui}=\lambda r_{ui} + (1-\lambda)\sqrt{ \frac{e^{s_{ui}}}{K}}$
  
  
  
%   \caption{Overall Training Process for AUR}
%   \label{train_process}
% \end{algorithm}
\subsection{Aleatoric Uncertainty}\label{sec:method-overall}%\vspace{-5pt}
% The label of implicit data is hard. 
In practical recommender systems, there are many potential positive samples that are blindly labeled as 0. When training on such data, a certain amount of useful information would be discarded, resulting in an ineffectively trained model.
% We need to quantify the likelihood that the sample will be mislabeled.
Therefore, it is an important task to quantify how likely a sample is mislabeled.
While traditional methods treat the recommendation problem as a homoscedastic regression task~\cite{2007Probabilistic}, in this work, we reformulate it as a heterogeneous regression problem where samples have different variances.

%As defined in %Section \ref{sec:problem}, 
%the problem formulation, we
We assume that the implicit feedback label $Y_{ui}$ follows the Gaussian Distribution $N(r_{ui},\sigma_{ui}^2)$, where $r_{ui}$ denotes the prediction of any recommendation model which is trained from the dataset $\mathcal{D}$.
%data described in Equation \eqref{label}. 
% Compared with traditional methods, they treat the problem as homoscedastic
The variance $\sigma_{ui}^2$ represents the stability of the Gaussian Distribution, which is a variable learned from the implicit data. 
A large variance $\sigma_{ui}^2$ usually indicates that the given label is unstable,
%. In other words,
\ie a label with large variance is likely to be incorrect.
%Therefore, it is natural to
We thus use the variance of the label to quantify the likelihood of mislabeling, which is referred to as aleatoric uncertainty.
% Similar to \cite{2017What}, we refine the recommendation problem as a heteroscedasticity problem. 
Similar to \cite{2017What}, we define the variance $\sigma_{ui}^2$ as our aleatoric uncertainty of the label $Y_{ui}$. 
% The log-likelihood of $Y_{ui}$ can be represented as:
% \begin{equation}
%     -logP(Y_{ui}|r_{ui},\sigma_{ui}^2)=\frac{(r_{ui}-Y_{ui})^2}{2\sigma_{ui}^2}+\frac{1}{2}log \ \sigma_{ui}^2.
% \end{equation}
% Due to the huge amount of training instances, we usually consider the mini-batch training strategy. In this work, instead of  randomly sampling $N$ \textit{user-item} pairs from a training set as a mini-batch, we adopt the same user-batch strategy used in \cite{liang2018variational}. We first randomly sample a batch of users $\mathcal{U}_{batch}$ from $\mathcal{U}$, then the user batch loss can be formulated as:
% \begin{equation}
% \begin{split}
% &L(\mathcal{U}_{batch},\mathcal{D};\theta,\phi)\\
% &=\sum_{u\in \mathcal{U}_{batch}, i \in \mathcal{I}}w_{ui}(\frac{(f_{\theta}(u,i)-Y_{ui})^2}{2g_{\phi}(u,i)}+\frac{1}{2}log \ g_{\phi}(u,i))+\Omega,
% \label{loss_overall}
% \end{split}
% \end{equation}
% where $w_{ui}$ denotes the weight of different samples in the training set $\mathcal{D}$, and $\Omega$ denotes the regularization term.
% % We will further introduce the specific training process in Section \ref{sec:training}. 
% This loss defines the overall learning objective. In the next subsection, we will introduce how to estimate the uncertainty.





\subsubsection{Uncertainty Estimator}\label{unestimator}
%As aforementioned, the backbone prediction $r_{ui}=f_{\theta}(u,i)$ is typically modeled with a neural network parameterized by $\theta$. 
%This subsection provides details on how to model the uncertainty $\sigma_{ui}^2$.
%Recall that the uncertainty is represented as the variance $\sigma_{ui}^2$, which is a non-negative variable.
We consider modeling the uncertainty $\sigma_{ui}^2$ in a similar manner as the backbone model $r_{ui}=f_{\theta}(u,i)$.
To ensure the non-negativity of $\sigma_{ui}^2$, we naturally consider denoting it by following the exponential form:
\begin{equation}\small
\sigma_{ui}^2=g_{\phi}(u,i)=\frac{e^{h_{\phi}(u, i)}}{K}.
\label{exponential}
\end{equation}
%The hyperparameter 
$K$ controls
%is used to control 
the scale of exponential function.
%In general, we set $K>1$.
%We will use \bm{$s_{ui}$} to denote the value of $h_{\phi}(u, i)$ in the rest of the paper. 
%
%Intuitively, users with similar item interactions should have similar uncertainty. 
% In this work, we do not consider any contextual features. 
%Therefore, we design an item-based modeling strategy.
Notice that the uncertainty of the label $Y_{ui}$ is a combination of the uncertainty signals from the user and item. 
We learn latent item representation $q_i$ and user representation $p_u$, similar to recommender models, and combine them as $h_{\phi}(u, i)$. 
%For each user-item pair $(u,i)$, we will model item representation $q_i$ and user representation $p_u$, respectively. Then, we combine them as $h_{\phi}(u, i)$. 
% For item $i$, the item-id vector $e_i$ denotes an one-hot vector whose $i_{th}$ element is equal to 1.
% We will learn an item encoder $$f_{item}:e_i \rightarrow q_i$$ to mine the feature of item itself.

As to item $i$, we learn a projection $f_{item}:e_i \rightarrow q_i$ to %mine the feature of item itself
mine the latent factors affecting uncertainty,
where $e_i$ denotes the one-hot encoding of item $i$.
For user representation, intuitively, users with similar item interactions should have similar uncertainty.
We employ the combination of all item representations in the user's historical interaction as the user representation. Formally,
%$i.e.$:
% $$p_u=\sigma(\frac{1}{\sqrt{|\mathcal{H}_u|}}\sum_{i\in \mathcal{H}_u}z_i),$$
$p_u=\sigma(\frac{1}{\sqrt{|\mathcal{H}_u|}}\sum_{i\in \mathcal{H}_u}z_i),$
where $\mathcal{H}_u$ denotes the historical interaction set of user $u$, and $\sigma$
indicates an activation function. $z_i$ is the user history information encoded by another projection\footnote{This design is similar to \cite{koren2008factorization}, which validates the rationality of using two different projections.} $f_{user}:e_i \rightarrow z_i$.
% For each item $i$ we learn two different embeddings $z_i$ and $q_i$, where $z_i$ is for encoding user history information and $q_i$ is for modeling features of the item itself. 
% We use $p_u$ to denote the embedding of user $u$, which is propagated from ${z_i| i \in H_u}$:
% \begin{equation}
% \begin{split}
% &p_u=\sigma(\frac{1}{\sqrt{|H_u|}}\sum_{i\in H_u}z_i) , where z_i=FFN_2(e_i)\\
% &q_i=FFN_1(e_i)\label{E9}
% \end{split}
% \label{embedding}
% \end{equation}
% Where $FFN_1$ and $FFN_2$ are two different feed-forward networks. $e_i$ denotes an one-hot vector whose $i_{th}$ element is equal to 0. $H_u$ denotes the historical interaction set of user u. $\sigma$ indicates an activation function. 
Then $h_{\phi}(u, i)$ is simply defined as the inner product of item representation $q_i$ and user representation $p_u$, \ie $h_{\phi}(u,i)=<p_u,q_i>$. For briefness, we denote the value of $h_{\phi}(u, i)$ as {$s_{ui}$} in the rest of the paper. 

%%TODO: add some sentences to end
% In the rest of papers, we will use $s_{ui}$  to denote the value of $g_{\phi}(u,i)$. 
% Besides directly controlling the scale, we assume that $s_{ui}$ has a zero-mean normal prior distribution.
% Similar to (\ref{expomf}), we also assume that the exposure indicator $a_{ui}$ has a fixed prior. 
% The overall assumption of uncertainty estimator is:
% \begin{equation}
% \begin{split}
% % &Loss=\alpha_1\sum_{(u,i)\in \textbf{O}}\frac{(r_{ui}-Y_{ui})^2}{e^{s_{ui}}}+\sum_{(u,i)\notin \textbf{O}}\frac{(r_{ui}-Y_{ui})^2}{e^{s_{ui}}}+\beta \sum_{u,i}s_{ui}+\gamma \sum_{u,i}s_{ui}^2\\
% % &\beta=k, \quad \gamma=\frac{k}{\tau^2}
% &s_{ui} \sim N(0,\tau^2)\\
% % &a_{ui} \sim Bernoulli(\frac{1}{\alpha_0})\\
% &Y_{ui} \sim N(r_{ui},\frac{e^{s_{ui}}}{k})\\
% \end{split}
% \end{equation}
% We then perform MAP inference in $Y_{ui}$. 
% \begin{equation}
% \begin{split}
% &\ \ \ \ E[-logP(Y|r_{ui},s_{ui})P(s_{ui})]\\
% &=E[-\frac{1}{mn}\sum_{u,i}a_{ui}(log\frac{1}{\sqrt{2\pi\sigma_{ui}^2}}e^{-\frac{(r_{ui}-Y_{ui})^2}{2\sigma_{ui}^2}}
% +log\frac{1}{\sqrt{2\pi\tau^2}}e^{-\frac{s_{ui}^2}{2\tau^2}})]\\
% &=\frac{1}{2mn}\sum_{u,i}E[a_{ui}](\frac{(r_{ui}-Y_{ui})^2}{ke^{s_{ui}}}+logke^{s_{ui}}+\frac{s_{ui}^2}{\tau^2})+c\\
% \end{split}
% \end{equation}
% we\ have\ E[a_{ui}]=1\ if\ (u,i) \in \textbf{O} \ else \  \frac{1}{\alpha_0} \\
% \end{split}
% \end{equation}
% where $c$ denotes a constant.Under above assumption,we have $E[a_{ui}]=1$ if $(u,i) \in \textbf{O}$ else $E[a_{ui}]=\frac{1}{\alpha_0}$. 
% After equivalent transformation, the final optimization objective can be reformulated as:
% \begin{equation}
% \begin{split}
% &L(U_{batch},D;\phi)=\sum_{u \in U_{batch},i}w_{ui}(\frac{(r_{ui}-Y_{ui})^2}{e^{s_{ui}}}+\beta s_{ui}+ \gamma s_{ui}^2)
% \label{loss}
% \end{split}
% \end{equation}
% where $\alpha,\beta,\gamma$ are hyper-parameters and $z_i,q_i (1\ge i\ge n)$ are learnable parameters. Note that while training the uncertainty estimator, the backbone model is expected to be well-trained and fixed. When making recommendations, we can directly recommend items with highest uncertainty. Inspired by the work in \cite{2009Risk}, the simple trade-off policy also improves the performance:
% \begin{equation}
% r_{ui}^{\prime}=(1-\lambda)r_{ui}+\lambda \sigma_{ui}^2
% \end{equation}
\subsection{Training Procedure}\label{sec:training}
%Since it's hard to learn the variance and expectation of a Normal Distribution at the same time for implicit data, we are better to train them separately.
A default choice for estimating the parameters of backbone model and uncertainty estimator is minimizing the negative log-likelihood of training samples. Formally, the negative log-likelihood of $Y_{ui}$ is $-logP(Y_{ui}|r_{ui},\sigma_{ui}^2)=\frac{(r_{ui}-Y_{ui})^2}{2\sigma_{ui}^2}+\frac{1}{2}log \ \sigma_{ui}^2$.
%can be represented as:
% \begin{equation}\small
%     -logP(Y_{ui}|r_{ui},\sigma_{ui}^2)=\frac{(r_{ui}-Y_{ui})^2}{2\sigma_{ui}^2}+\frac{1}{2}log \ \sigma_{ui}^2.
% \end{equation}
Due to the huge amount of training instances, we usually consider the mini-batch training strategy. 
%Instead of randomly sampling $N$ \textit{user-item} pairs 
%from a training set 
%as a mini-batch, we
We adopt the same user-batch strategy used in \cite{liang2018variational}. We first randomly sample a batch of users $\mathcal{U}_{batch}$ from $\mathcal{U}$, then the user batch loss $L(\mathcal{U}_{batch},\mathcal{D};\theta,\phi)$ can be formulated as:
% \begin{equation}
% \begin{split}
% &L(\mathcal{U}_{batch},\mathcal{D};\theta,\phi)\\
% &=\sum_{u\in \mathcal{U}_{batch}, i \in \mathcal{I}}w_{ui}(\frac{(f_{\theta}(u,i)-Y_{ui})^2}{2g_{\phi}(u,i)}+\frac{1}{2}log \ g_{\phi}(u,i))+\Omega,
% \label{loss_overall}
% \end{split}
% \end{equation}
% \begin{equation}
% \begin{split}
% &L(\mathcal{U}_{batch},\mathcal{D};\theta,\phi)\\
% &=\sum_{u\in \mathcal{U}_{batch}, i \in \mathcal{I}}w_{ui}\left(
%     \frac{(r_{ui}-Y_{ui})^2}{
%         \frac{2}{K}e^{s_{u,i}}}+\frac{1}{2} \ s_{u,i}
% \right)+\Omega,
% \label{loss_overall}
% \end{split}
% \end{equation}
\begin{equation}\small
\begin{split}
\sum_{u\in \mathcal{U}_{batch}, i \in \mathcal{I}}w_{ui}\left(
    \frac{(r_{ui}-Y_{ui})^2}{
        \frac{2}{K}e^{s_{u,i}}}+\frac{1}{2} \ s_{u,i}
\right)+\Omega,
\label{loss_overall}
\end{split}
\end{equation}
where $w_{ui}$ denotes the weight of different samples in the training set $\mathcal{D}$, and $\Omega$ denotes the regularization term.

% We will further introduce the specific training process in Section \ref{sec:training}. 
%This loss defines the overall learning objective. In the next subsection, we will introduce how to estimate the uncertainty.

% Learning both the variance and the expectation of a Normal Distribution simultaneously, from the implicit data, is unstable. In this work, 
Noticing that optimizing the two models simultaneously can lead to unstable issues and overfitting~\cite{yu2020sampler},
we propose to train them sequentially in an Expectation-Maximization like algorithm. In particular, we first train the backbone model as our expectation estimator without considering the uncertainty, and then train the uncertainty estimator while fixing the expectation model. 
%Moreover, in industry applications, retraining the original backbone model together with the uncertainty model is usually time consuming and expensive. 
% We will also show the results of the joint learning of expectation and uncertainty in the experiments.
%Therefore, it's important to train the uncertainty estimator only based on the prediction values of backbone models.
Sequential training also simulates the situation where our method is grafted onto an existing model, which is required by industry applications. We also show the results of the joint learning of expectation and uncertainty in the experiments (\cf Table~\ref{variant}).
\begin{algorithm}[h]
  \SetAlgoLined
  \KwData{Hyperparameters $K$,$\alpha$,$\beta$,$\gamma$,$\lambda$,$\mu$}
  \KwResult{Fixed prediction $Pred_{ui}$ for each (u,i) }
  initialization $\theta$, $\Phi$\;
  \textbf{Backbone Training Process}\;
  \While{not converge }{
  for each (u,i) $r_{ui}=f_{\theta}(u,i)$\;
  Update parameter $\theta$ by Equation \ref{loss_backbone}\;
  }
  \textbf{Uncertainty Estimator Training Process}\;
  \While{not converge }{
  for each (u,i) $r_{ui}=f_{\theta}(u,i)$\;
  for each (u,i) $s_{ui}=h_{\phi}(u,i)$\;
  Update parameter $\phi$ by Equation \ref{loss}\;
  }
  Fix the original model prediction by aleatoric uncertainty $Pred_{ui}=\lambda r_{ui} + (1-\lambda)\sqrt{ \frac{e^{s_{ui}}}{K}}$
  
  
  
  \caption{Overall Training Process for AUR}
  \label{train_process}
\end{algorithm}
% \subsubsection{Backbone Model Training}


%\subsubsection{Expectation Estimator Training}\label{expectation_training}
\subsubsection{Backbone Training}\label{expectation_training}
% We directly take a backbone recommender model as our expectation estimator. To train a sample but strong expectation estimator, we need considering the extremely imbalance distribution between positive and negative samples. Thus, we decide to leverage a sampling strategy to mitigate the unbalanced problem. For each sample (u,i), we define its sampling probability as:
%We train a backbone model as our expectation estimator. 
%In our training set, the positive samples and negative samples are severely imbalanced. 
%In order to obtain strong backbone model, we decide to leverage the sampling strategy. 
To alleviate the imbalance issue of positive and negative samples, we leverage a sampling strategy.
We assign the weight to each instance $w_{ui}$ as follows:
\begin{equation}\small
    w_{ui}\sim
   \begin{cases}
   1 &\mbox{$Y_{ui}=1$,}\\
   Bernoulli(\mu) &\mbox{$Y_{ui}=0$.}
   \end{cases}
   \label{weight}
\end{equation}
where $\mu$ denotes the sampling rate for negative samples.
% High $\mu$ indicates the negative samples are important for backbone model training.
% The sampling strategy reduces the weight of negative samples indirectly and improves the performance. In our experiments, we also verify that the model trained by minimizing square error with this strategy outperforms the original BPR \cite{2009BPR} strategy. 
% We have verified that it's hard to learn the variance and expectation of a Normal Distribution. 
% We will first train the expectation model and then train the variance model. 
% This also simulates the situation where our method is grafted onto an existing model.
The aleatoric uncertainty is not considered for the backbone model,  
%$g_{\phi}(u,i)=1$
$s_{ui}$ is thus fixed for all users and items. 
%The second term in Equation (\ref{loss_overall}) is equal to 0, and we only need to minimize over the first regression term and the third regularization, \ie $\Omega=\lambda||\theta||^2$.
We set $s_{ui} = 0$ and use $l_2$-norm as regularization, \ie $\Omega=\lambda||\theta||^2$, simplifying the training objective for backbone model as:
%The training objective for backbone model can be simplified as:
\begin{equation}\small
\begin{split}
&L(\mathcal{U}_{batch},\mathcal{D};\theta)=\sum_{u\in \mathcal{U}_{batch}, i \in \mathcal{I}}w_{ui}\left(
    \frac{(r_{ui}-Y_{ui})^2}{2}
\right)+\lambda ||\theta||^2.
\label{loss_backbone}
\end{split}
\end{equation}
%In this work, we trained MF, LightGCN, and MultiVAE to be our backbone models.
%The sampling strategy reduces the weight of negative samples indirectly and improves the performance. 
%Note that the 
The first term is essentially a mean square error, one of the common recommendation losses. 
%Actually, the
The form of the loss is decided by the prior assumption of data distribution. Other losses like BPR \cite{2009BPR} corresponds to distributions other than Gaussian Distribution.
%In this work, we find that our objective 
We belief Gaussian Distribution is a reasonable assumption since Equation ~\eqref{loss_backbone} can lead to stronger backbone models than BPR (\cf Figure~\ref{fair}).
%we trained MF, LightGCN, and MultiVAE to be our backbone models by minimizing Equation~\ref{loss_backbone}
%In our experiments, we also verify that the model trained by minimizing square error with this strategy outperforms the original BPR \cite{2009BPR} strategy. 

% We briefly review ExpoMF \cite{2016Modeling} and give a simplified variant as backbone model.    

% ExpoMF is a famous improved version of matrix factorization for implicit data, which assigns adaptive exposure prior probability to each user-item pair. 
% More generally, we reformulate the assumptions in ExpoMF as:
% \begin{equation}
% \begin{split}
% &\theta \sim N(0,\sigma_0^2 \textbf{I})\\ 
% &a_{ui} \sim Bernoulli(\mu_{ui})\\
% &Y_{ui}|a_{ui}=1 \sim N(f_{\theta}(u,i), \sigma_1^2)\\
% &Y_{ui}|a_{ui}=0 \sim \delta_0
% \label{expomf}
% \end{split}
% \end{equation}
% where $a_{ui}$ indicates whether item i is exposed to user, and $\delta_0$ indicates that $P(Y_{ui}=1|a_{ui}=0)=0$. 
% For an unobserved (u,i) pair, if $r_{ui}$ is high,  $\mu_{ui}$ would be forced to 0 which denotes that the item $i$ is very likely to be not exposed to user $u$.
% In our work, we simplify the estimation of exposure prior by assigning a fixed hyper-parameter $\alpha$ to all (u,i) pairs. It is to say that $a_{ui} \sim Bernoulli(\alpha)$. The overall optimization objective of backbone model for the batch of users is formulated as :
% \begin{equation}
% \begin{split}
%     L(U_{batch},D;\theta)=\sum_{u\in U_{batch}, i \in \textbf{I}}a_{ui}(f_{\theta}(u,i)-Y_{ui})^2+\lambda||\theta||^2
% \end{split}
% \end{equation}
% where $\lambda$ denotes the hyper-parameter to control the regularization term. In this work, we treat MF, LightGCN, and MultiVAE as our backbone models.
\subsubsection{Uncertainty Estimator Training}
The uncertainty estimator is trained on top of the backbone model. In this stage, we also need to balance the positive and negative samples, although the learning objective is not the hard label of implicit data. 
To speed up training, we replace the sampling process by directly assigning fixed weight to each instance.
The weight $w_{ui}$ there can be formulated as:
\begin{equation}\small
    w_{ui}=
   \begin{cases}
   \alpha &\mbox{$Y_{ui}=1$,}\\
   1 &\mbox{$Y_{ui}=0$.}
   \end{cases}
   \label{weight}
\end{equation}
where $\alpha$ is a key hyperparameter for training the uncertainty estimator. More specifically, $\alpha$ can be adjusted to control the strength of 
%improving
emphasizing the tail items (\cf Figure~\ref{hyper}). 
%We refer to $\alpha$ as \textbf{tail-controlling ratio}.

To optimize the uncertainty estimator, we first derive the distribution of uncertainty $P(s_{ui}|r_{ui},Y_{ui})$. According to Bayes theorem, we can get:
\begin{equation}\small
    P(s_{ui}|r_{ui},Y_{ui})=\frac{P(Y_{ui}|r_{ui},s_{ui})P(r_{ui}|s_{ui})P(s_{ui})}{P(r_{ui},Y_{ui})}.
\end{equation}
Since the expectation and variance of a Gaussian Distribution are independent statistics~\cite{casella2021statistical}, $s_{ui}$ and $r_{ui}$ are independent. We have $P(r_{ui}|s_{ui})=P(r_{ui})$. Note that when training the uncertainty estimator, $r_{ui}$ is fixed and treated as a constant. Then we have $P(s_{ui}|r_{ui},Y_{ui}) \propto P(Y_{ui}|r_{ui},s_{ui})P(s_{ui})$. We assume that $s_{ui}$ has a prior of zero-mean Gaussian Distribution: $s_{ui} \sim N(0,\tau^2)$.
Combined with Equation \eqref{exponential}, we obtain the posterior probability of $s_{ui}$ and minimize its negative logarithm to optimize the parameters of uncertainty estimator. Formally,
%is formulated as:
\begin{equation}\small
    -logP(s_{ui}|r_{ui},Y_{ui})=\frac{(r_{ui}-Y_{ui})^2}{\frac{2}{K}e^{s_{ui}}}+\frac{1}{2}s_{ui}+\frac{s_{ui}^2}{\tau^2}+c,
\end{equation}
% Different from backbone model training, the regularization term is set to punish $h_{\phi}(u,i)$. As in equation (\ref{loss}), the regularization there can be formulated as:
% \begin{equation}
%     \Omega=\lambda \sum_{u\in U_{batch},i}(h_{\phi}(u,i))^2
% \end{equation}
% Note that we fix the expectation $r_{ui}$ during the training of $\sigma_{ui}^2$,  
where $c$ denotes a constant. After simplifying the form, the final optimization objective is:
\begin{small}
\begin{equation}
\begin{split}
&L(\mathcal{U}_{batch},\mathcal{D};\phi)=\sum_{u \in \mathcal{U}_{batch},i \in \mathcal{I}}w_{ui}\left(
    \frac{(r_{ui}-Y_{ui})^2}{e^{s_{ui}}}+\beta s_{ui}+ \gamma s_{ui}^2
\right),
\label{loss}
\end{split}
\end{equation}
\end{small}
where $\beta$, $\gamma$ are hyperparameters.
This training process can be understood as finding the best variances such that the data likelihood is maximized.

After obtaining the optimal values of the variance, our model makes recommendations based on both of the expectation and aleatoric uncertainty. The overall training process is organized as Algorithm \ref{train_process}.
% \begin{equation}
% Pred_{ui}=(1-\lambda)r_{ui}+\lambda \sigma_{ui}
% \end{equation}
% \textcolor{red}{
$Pred_{ui}$ denotes the final prediction of the pair $(u,i)$. 
Given the pair $(u,i)$, the final prediction is $Pred_{ui}=(1-\lambda)r_{ui}+\lambda \sigma_{ui}$.
When $\lambda = 0 $, the prediction degenerates to the backbone model.
% }

% \textbf{After obtaining the optimal values of the variance, our model makes recommendations based on the uncertainty, where a user-item pair with larger uncertainty will be ranked higher}.
% \subsection{Uncertainty Estimator}\label{sec:estimator}
 
% In this section, we will introduce how to model the uncertainty in detail.
% We treat the variance $\sigma_{ui}^2$ as uncertainty.
% The variance $\sigma_{ui}^2$ should be a non-negative variable.
% To ensure the learnable parameters $\sigma_{ui}^2>0$, we naturally consider to leverage an exponential function :
% \begin{equation}
% \sigma_{ui}^2=g_{\phi}(u,i)=\frac{e^{h_{\phi}(u,i)}}{k}
% \label{E8}
% \end{equation}
% where $k$ is used to control the scale of exponential function. In general, we need to set $k>1$.
% In the rest of the paper, we will use $s_{ui}$  to denote the value of $g_{\phi}(u,i)$. 
% In this work, we do not consider any contextual features. 
% Therefore, in order to better mine the information of historical interactions, we design an item-based modeling strategy. For each item $i$ we learn two different embeddings $z_i$ and $q_i$, $z_i$ is for encoding user history information and $q_i$ is for modeling features of the item itself. We use $p_u$ to denote the embedding of user $u$, which is propagated from ${z_i}_{i \in H_u}$. 
% The detail is formulated as:
% \begin{equation}
% \begin{split}
% &p_u=\sigma(\frac{1}{\sqrt{|H_u|}}\sum_{i\in H_u}z_i)\\
% &q_i=FFN_1(e_i) , z_i=FFN_2(e_i)\label{E9}
% \end{split}
% \end{equation}
% Where $FFN_1$, $FFN_2$ denote two different feed-forward network ,$e_i$ denotes an one-hot vector whose $i_{th}$ element is equal to 0, and $H_u$ denotes the historical interaction set of user u. $\sigma$ indicates an activation function. 
% Then, $h_{\phi}$ is simply defined as the inner product of the pair of embedding:
% \begin{equation}
% h_{\phi}(u,i)=<p_u,q_i>\label{E10}
% \end{equation}

% % In the rest of papers, we will use $s_{ui}$  to denote the value of $g_{\phi}(u,i)$. 
% Besides directly controlling the scale, we assume that $s_{ui}$ has a zero-mean normal prior distribution.
% % Similar to (\ref{expomf}), we also assume that the exposure indicator $a_{ui}$ has a fixed prior. 
% The overall assumption of uncertainty estimator is:
% \begin{equation}
% \begin{split}
% % &Loss=\alpha_1\sum_{(u,i)\in \textbf{O}}\frac{(r_{ui}-Y_{ui})^2}{e^{s_{ui}}}+\sum_{(u,i)\notin \textbf{O}}\frac{(r_{ui}-Y_{ui})^2}{e^{s_{ui}}}+\beta \sum_{u,i}s_{ui}+\gamma \sum_{u,i}s_{ui}^2\\
% % &\beta=k, \quad \gamma=\frac{k}{\tau^2}
% &s_{ui} \sim N(0,\tau^2)\\
% % &a_{ui} \sim Bernoulli(\frac{1}{\alpha_0})\\
% &Y_{ui} \sim N(r_{ui},\frac{e^{s_{ui}}}{k})\\
% \end{split}
% \end{equation}
% % We then perform MAP inference in $Y_{ui}$. 
% % \begin{equation}
% % \begin{split}
% % &\ \ \ \ E[-logP(Y|r_{ui},s_{ui})P(s_{ui})]\\
% % &=E[-\frac{1}{mn}\sum_{u,i}a_{ui}(log\frac{1}{\sqrt{2\pi\sigma_{ui}^2}}e^{-\frac{(r_{ui}-Y_{ui})^2}{2\sigma_{ui}^2}}
% % +log\frac{1}{\sqrt{2\pi\tau^2}}e^{-\frac{s_{ui}^2}{2\tau^2}})]\\
% % &=\frac{1}{2mn}\sum_{u,i}E[a_{ui}](\frac{(r_{ui}-Y_{ui})^2}{ke^{s_{ui}}}+logke^{s_{ui}}+\frac{s_{ui}^2}{\tau^2})+c\\
% % \end{split}
% % \end{equation}
% % we\ have\ E[a_{ui}]=1\ if\ (u,i) \in \textbf{O} \ else \  \frac{1}{\alpha_0} \\
% % \end{split}
% % \end{equation}
% % where $c$ denotes a constant.Under above assumption,we have $E[a_{ui}]=1$ if $(u,i) \in \textbf{O}$ else $E[a_{ui}]=\frac{1}{\alpha_0}$. 
% After equivalent transformation, the final optimization objective can be reformulated as:
% \begin{equation}
% \begin{split}
% &L(U_{batch},D;\phi)=\sum_{u \in U_{batch},i}w_{ui}(\frac{(r_{ui}-Y_{ui})^2}{e^{s_{ui}}}+\beta s_{ui}+ \gamma s_{ui}^2)
% \label{loss}
% \end{split}
% \end{equation}
% $\alpha,\beta,\gamma$ are hyper-parameters and $z_i,q_i (1\ge i\ge n)$ are learnable parameters. While training the uncertainty estimator, the backbone model is expected to be well-trained and fixed. When we make recommendations, we can directly recommend items with highest uncertainty. Inspired by \cite{2009Risk}, the simple trade-off policy also improves the performance:
% \begin{equation}
% r_{ui}^{\prime}=(1-\lambda)r_{ui}+\lambda \sigma_{ui}^2
% \end{equation}
%%%follow pic is need
\begin{figure}[t]
	\centering
	%\subfigbottomskip=1pt
	\subfigure{
		\includegraphics[width=0.44\columnwidth]{pic/sigma_r_Yelp.png}
	}
	\subfigure{
		\includegraphics[width=0.44
		\columnwidth]{pic/sigma_r_Amazon.png}
	}
 	\vspace{-10pt}
	\caption{Relationship between $r_{ui}^2$ and $\sigma_{ui}^2$.}
	\vspace{-10pt}
\label{r_sigma}
\end{figure}


\subsection{Theoretical Analysis}\label{sec:algo}
In this subsection, we first show that the overall performance of the recommendation with aleatoric uncertainty is at least as good as the backbone models using expectation. The statement is further verified empirically with results from two real datasets (\cf Table~\ref{main result}). We then explain the mechanism of improving the tail performance.
%\subsubsection{Overall Performance}

\noindent \textbf{$\bullet$ Overall Performance. }
We first state the property that connects the aleatoric uncertainty with the expectation. 
% \begin{theorem}
% Denote the residual of the expectation as $\Delta_{ui}=r_{ui}-Y_{ui}$. The uncertainty is represented as $e^{s_{ui}}/K$ in Equation (\ref{exponential}). For simplicity, assume the weights $w_{ui}$ are the same for all user-item pairs. For an user $u$, denote the distributions of $\Delta_{ui}^2$ and $e^{s_{ui}}/K$ over the items as $p_u$ and $q_u$ respectively. Then the following inequality holds:
% \begin{equation}
%     L(\mathcal{D}) \ge \sum_{u}KL(p_{u}||q_{u}) + c
% \end{equation}
% here $L(\mathcal{D})$ is the loss of uncertainty estimator in Equation (\ref{loss}). $KL(p_u||q_u)$ is the KL-Divergence of the two distributions. $c$ is constant. 
% \end{theorem}
\begin{theorem}
Denote the residual of the expectation as $\Delta_{ui}=r_{ui}-Y_{ui}$. 
%The uncertainty is represented as $e^{s_{ui}}/K$ in Equation (\ref{exponential}). For simplicity, assume the weights $w_{ui}$ are the same for all user-item pairs. 
For user $u$, denote the distributions of $\Delta_{ui}^2$ and $e^{s_{ui}}/K$ over the items as $p_u$ and $q_u$ respectively.
If the weights $w_{ui}$ are the same for all user-item pairs, the following inequality holds:
\begin{equation}\small
    L(\mathcal{D}) \ge \sum_{u}KL(p_{u}||q_{u}) + c,
\end{equation}
where $L(\mathcal{D})$ is the loss of uncertainty estimator in Equation \eqref{loss}; $KL(p_u||q_u)$ is the KL-Divergence of the two distributions; and $c$ is a constant. 
\end{theorem}

\textbf{Proof of Theorem 1}\label{proof}
The training objective of uncertainty estimator, \ie Equation (\ref{loss}) can be written as:
\begin{equation}
\small
\begin{split}
&L(D)=\sum_u\sum_{i}(\frac{\Delta_{ui}^2}{e^{s_{ui}}}+\beta s_{ui}+ \gamma s_{ui}^2)
\end{split}
\end{equation}
here we assume $w_{ui}$ or $\alpha$ in equation (\ref{weight}) is 1, but it is trivial to obtain a similar inequality for $\alpha \neq 1$.
We obtain the normalized distribution of $p_u$ and $q_u$ as $p_{ui}= \frac{\Delta_{ui}^2}{K_{u}}$ and $q_{ui}=\frac{e^{s_{ui}}}{R_{u}}$,
% \begin{equation}
% \begin{split}
% &p_{ui}= \frac{\Delta_{ui}^2}{K_{u}} \quad
% q_{ui}=\frac{e^{s_{ui}}}{R_{u}}
% \end{split}
% \end{equation}
where $K_{u}=\sum_{i}\Delta_{ui}^2, R_{u}=\sum_{i}e^{s_{ui}}$, and $p_{ui}$ and $q_{ui}$ denote the value of $p_u$ and $q_u$ on the $i$-$th$ item.
According to the common inequality: $lnx+1 \le x (x>0)$, we can derive the inequality:
\begin{equation}
\small
    \frac{\Delta_{ui}^2}{e^{s_{ui}}}=  \frac{\Delta_{ui}^2}{K_{u}}\frac{K_{u}}{e^{s_{ui}}}\ge \frac{\Delta_{ui}^2}{K_{u}}(ln\frac{\frac{\Delta_{ui}^2}{K_{u}}}{\frac{e_{s_{ui}}}{R_{u}}}+ln\frac{K_{u}^2}{R_{u}}+1-ln\Delta_{ui}^2)
\end{equation}
By substituting the above inequality into $L(D)$, we have:
%can obtain:
\begin{equation}\small
\begin{split}
&L(\mathcal{D})\ge \sum_{u}\sum_{i}(p_{ui}(ln\frac{p_{ui}}{q_{ui}}-lnR_{u})+\beta s_{ui}+ \gamma s_{ui}^2)+c_1\\
&=\sum_{u}KL(p_{u}||q_{u})+\sum_{u}\sum_{i}(\beta s_{ui}+ \gamma s_{ui}^2 -lnR_{u})+c_1
\end{split}
\label{eq21}
\end{equation}
Assume that $s_{uk}=max_{i}s_{ui}$, we have $lnR_{u}\le ln|\mathcal{I}|e^{s_{uk}}=s_{uk}ln|\mathcal{I}|$ and $\mathcal{I}$ is the set of all items. According to the Extremum Theorem of a quadratic function, we can derive:
\begin{equation}
\begin{split}
&\beta s_{ui}+ \gamma s_{ui}^2 \ge \frac{-\beta ^2}{4\gamma} \ \ \ \ \ \ \  for \ i \neq k\\
&(\beta-ln|\mathcal{I}|) s_{uk}+\gamma s_{uk}^2 \ge \frac{-(\beta-ln|\mathcal{I}|) ^2}{4\gamma} \ for \ i = k
\end{split}
\end{equation}
Therefore, the second term in the RHS of the inequality (\ref{eq21}) is also lower bounded by a constant.
Overall, we can obtain the inequality:
\begin{equation}
\small
    L(\mathcal{D}) \ge \sum_{u}KL(p_{u}||q_{u})+c
\end{equation}
This completes the proof of the theorem.\quad


The above theorem essentially states that the KL-Divergence between the distributions of expectation and uncertainty is bounded by the loss function that is being optimized. In other words, the lower the loss can be achieved, the closer the two distributions will become. Therefore, the expectation and the uncertainty are highly positively correlated, and thus the overall performance of uncertainty recommendation should be at least on par with the recommendation models using expectation. 


% \begin{table}[]
% \caption{The expectation and uncertainty of selected users}
% \begin{tabular}{ccccc}
% \hline
%               & i_1   & i_2   & i_3   & i_4   \\ \hline
% Expectation   & 0.8038 & 0.7784 & 0.7654 & 0.4648 \\ \hline
% Uncertainty   & 0.3188 & 0.2952 & 0.3050 & 0.3277 \\ \hline
% Popularity    & 128    & 44     & 59     & 40     \\ \hline
% User Feedback & 0      & 0      & 0      & 1      \\ \hline
% \end{tabular}
% \label{pop}
% \end{table}
% \begin{table}
% \small
% \caption{Case study of selected user-items.}
% \begin{tabular}{|c|cccc|}
% \hline
% Items         & i\_1   & i\_2   & i\_3   & i\_4   \\ \hline
% Expectation   & 0.8038 & 0.7784 & 0.7654 & 0.4648 \\
% Uncertainty   & 0.3188 & 0.2952 & 0.3050 & 0.3277 \\
% Popularity    & 128    & 44     & 59     & 40     \\
% User Feedback & 0      & 0      & 0      & 1      \\ \hline
% \end{tabular}
% \label{pop}
% \end{table}
To further validate the above statement, we report the empirical results on two real world datasets in Figure \ref{r_sigma}. Specifically, we randomly select one user from each dataset and show the visual relationship between $r_{ui}^2$ and $\sigma_{ui}^2$. 
%After sorting the expectation $r_{ui}$ in order, we draw the variance/uncertainty $\sigma_{ui}^2$ corresponding to each $r_{ui}^2$.
As shown in Figure \ref{r_sigma}, it is clear that expectation and uncertainty have strong linear positive correlation for both users, which confirms the theorem. The yellow line indicates the best fit line. Moreover, we calculate the mean pearson correlation coefficient on different datasets over the users, where it is 0.69 on Amazon-Book and 0.74 on Yelp (see dataset descriptions in Section \ref{ssec:exp_setting}).

%\subsubsection{Tail Performance}\label{tail discuss}
\noindent \textbf{$\bullet$ Tail Performance. }
We also claim that using uncertainty to make recommendations improves the quality of tail items recommendations. 
The reason is that when a positive sample is not able to be retrieved by the expectation $r_{ui}$, its variance $\sigma_{ui}^2$ would be learned to be a large value. 
%In this case, this
This positive sample is likely to be captured by our AUR model. Especially, when the hyperparameter $\alpha$ in Equation \eqref{weight} increases, the $\sigma_{ui}^2$ of tail items would also increase. Therefore, we name $\alpha$ as the \textbf{tail-controlling coefficient}.

We use an example to illustrate this statement in Table \ref{pop}. We select a user and four items from the Amazon-Book dataset to compare the learned expectations and uncertainties. The backbone model is MF. We count item popularity in the training set while the user feedback is retrieved from the testing set. From the table, we can see that $i_4$ has a much lower popularity compared to $i_1$, as well as its expectation.
%However, the uncertainty of $i_4$ is higher than $i_1$.
Despite that item $i_1$ has been interacted many times, it is actually a true negative sample for the user.
%On the other hand, both
Both the popularity and the expectation of $i_4$, a true positive sample, are the lowest among the four items, but it still has the highest uncertainty indicating that $i_4$ is a potential positive sample. We provide more analysis in the experiments.
\begin{table}
\small
\centering
\caption{Case study of selected user-item pairs. We show four items with their expectation, uncertainty, and popularity in Amazon to explain how AUR improves the tail performance. }
\vspace{-4mm}
\begin{tabular}{|c|cccc|}
\hline
Items         & $i_1$   & $i_2$   & $i_3$   & $i_4$   \\ \hline
Expectation   & 0.8038 & 0.7784 & 0.7654 & 0.4648 \\
Uncertainty   & 0.3188 & 0.2952 & 0.3050 & 0.3277 \\
Popularity    & 128    & 44     & 59     & 40     \\
User Feedback & 0      & 0      & 0      & 1      \\ \hline
\end{tabular}
\label{pop}
\vspace{-6mm}
\end{table}



\subsection{Discussion}\label{sec:discussion}
%\subsubsection{Relevance to Sample Weighting}
\noindent \textbf{$\bullet$ Relevance to Sample Weighting. }
% This subsection provides discussion that connects our approach with previous methods as well as their distinctions.
We first discuss the connections and distinctions between our approach and previous methods. 
In the previous discussion, \cite{2009Collaborative,reweight1} heuristically assigned weights $c_{ui}$ to each training sample. In our work, if we fix $s_{ui}=log(\frac{1}{c_{ui}})$ and $\alpha=1$ in Equation \eqref{loss} to optimize the backbone model, our approach is equivalent to \cite{2009Collaborative,reweight1}.
Intuitively, for the positive samples, high correlation between $(u,i)$ indicates low variance \cite{2009Collaborative}. For the negative samples, high correlation indicates that the item $i$ might be a potential positive sample for user $u$, resulting in a high variance \cite{reweight1}.
Therefore, assigning fixed weights to re-weight MSE loss in the training process is essentially to determine the uncertainty of each sample.
% For the observed samples, higher confidence $c_{ui}$ means the lower uncertainty.
% There are several major differences between our approach and previous methods. 
Previous methods specify/fix the variance to learn the expectation. In contrast, our approach first learns an expectation, and then estimates the variance based on the learned expectation. During the recommendation stage, previous methods recommend items using expectation while we make recommendations with variance to better capture the uncertainty in the data.
% \subsubsection{Relevance to Probabilistic Recommender Methods}

\noindent \textbf{$\bullet$ Relevance to Probabilistic Methods. }
Similar to AUR, some probabilistic models, \textit{e.g.}, PMF \cite{2007Probabilistic} and ExpoMF \cite{2016Modeling}, also assume the implicit labels obey Gaussian Distributions. Differently, they take the variances of Gaussian Distributions as hyper-parameters, and assume all $(u,i)$ pairs have the same variances. 
%These models thus consider fixed and coarse-grained uncertainty. 
%On the contrary, 
AUR estimates the variances for each $(u,i)$ pair with the proposed learning strategy, obtaining more accurate uncertainties at a fine-grained user-item pair level.
%Similar to the famous probabilistic models PMF \cite{2007Probabilistic} and ExpoMF \cite{2016Modeling}, our AUR framework also assumes that the labels obey Gaussian distribution. They assume that the labels $Y_{ui}$, the user embeddings $e_u$, and the item embeddings $e_i$ obey three different Gaussian distributions $N(\langle e_u,e_i\rangle,\lambda^{-1}_Y), N(0,\lambda^{-1}_U \textbf{I}), N(0,\lambda^{-1}_I \textbf{I})$ respectively, where $\lambda^{-1}_Y$, $\lambda^{-1}_U$, and $\lambda^{-1}_I$ are fixed as hyper-parameters. Essentially, they provide fixed and coarse-grained uncertainty to better capture the predicted expectations. Our AUR framework estimates the fine-grained uncertainty on each $(u,i)$ pair by learning strategy, which is much more detailed and exact. '=
Moreover, these probabilistic models generate recommendations with the predicted expectations, which may over-recommend popular items,as discussed in Section~\ref{exp_prob}. Fundamentally different to them, AUR makes recommendations based on the uncertainties, aiming at providing more accurate and more balanced recommendations.
% Besides, when serving, these probabilistic methods generate recommendations which are only depend on the predicted expectations. However, as discussed before, the predicted expectations tend to recommend excessive popular items. Therefore, our AUR framework makes recommendations based on the uncertainties but not the expectations, which can provide more accuracy and more balance recommendations. 

==> method_rivise.tex <==
\section{METHOD}\label{sec:method}
\textbf{Problem Formulation. }
% Suppose we have an implicit 
% feedback dataset 
% $\mathcal{D}$ with $m$ users and $n$ items. The set of users and items are represented as $\mathcal{U}$ and $\mathcal{I}$. 
% For any $u \in \mathcal{U}$ and $i \in \mathcal{I}$, the label of pair $(u,i)$ is $Y_{ui}=1$, if $u$ has consumed $i$, and $Y_{ui}=0$ otherwise.
% Let $\mathcal{R}=\{ r_{ui} \}_{m \times n}$ denotes the prediction given by a 
% backbone model (\eg MF) parameterized with $\theta$, \ie $r_{ui}=f_{\theta}(u,i)$.
% We assume that $Y_{ui} \sim N(r_{ui},\sigma_{ui}^2)$ and learn the variance $\sigma_{ui}^2$ as our aleatoric uncertainty. 
% The backbone prediction and uncertainty estimation can be represented as $r_{ui}=f_{\theta}(u,i)$ and $\sigma_{ui}^2=g_{\phi}(u,i)$, where $g_{\phi}(\cdot, \cdot)$ denotes the uncertainty estimator parameterized with $\phi$. 
% The overall training process is organized as Algorithm \ref{train_process}.
Consider a scenario where we have a dataset $\mathcal{D}$ consisting of implicit feedback, with $m$ users and $n$ items. The set of users and items are represented as $\mathcal{U}$ and $\mathcal{I}$ respectively. For any user $u$ in $\mathcal{U}$ and item $i$ in $\mathcal{I}$, the label of the pair $(u,i)$ is represented as $Y_{ui}$, where $Y_{ui}=1$ if user $u$ has consumed item $i$, and $Y_{ui}=0$ otherwise. We utilize a backbone model, for instance, Matrix Factorization (MF), parameterized with $\theta$, to make a prediction denoted as $\mathcal{R}=\{ r_{ui} \}_{m \times n}$, such that $r_{ui}=f_{\theta}(u,i)$. We assume that $Y_{ui}$ follows a normal distribution with mean $r_{ui}$ and a variance $\sigma_{ui}^2$, where we learn the variance $\sigma_{ui}^2$ as our aleatoric uncertainty. The prediction $r_{ui}$ and the uncertainty estimate $\sigma_{ui}^2$ can be represented as $r_{ui}=f_{\theta}(u,i)$ and $\sigma_{ui}^2=g_{\phi}(u,i)$ respectively, where $g_{\phi}(\cdot, \cdot)$ represents the uncertainty estimator parameterized with $\phi$. The training process is organized as Algorithm \ref{train_process}.

\begin{algorithm}[h]
  \SetAlgoLined
  \KwData{Hyperparameters $K$,$\alpha$,$\beta$,$\gamma$,$\lambda$,$\mu$}
  \KwResult{Fixed prediction $Pred_{ui}$ for each (u,i) }
  initialization $\theta$, $\Phi$\;
  \textbf{Backbone Training Process}\;
  \While{not converge }{
  for each (u,i) $r_{ui}=f_{\theta}(u,i)$\;
  Update parameter $\theta$ by Equation \ref{loss_backbone}\;
  }
  \textbf{Uncertainty Estimator Training Process}\;
  \While{not converge }{
  for each (u,i) $r_{ui}=f_{\theta}(u,i)$\;
  for each (u,i) $s_{ui}=h_{\phi}(u,i)$\;
  Update parameter $\phi$ by Equation \ref{loss}\;
  }
  Fix the original model prediction by aleatoric uncertainty $Pred_{ui}=\lambda r_{ui} + (1-\lambda)\sqrt{ \frac{e^{s_{ui}}}{K}}$
  
  
  
  \caption{Overall Training Process for AUR}
  \label{train_process}
\end{algorithm}

\subsection{Aleatoric Uncertainty}\label{sec:method-overall}
% In practical recommender systems, there are many potential positive samples that are blindly labeled as 0. When training on such data, a certain amount of useful information would be discarded, resulting in an ineffectively trained model.
% Therefore, it is an important task to quantify how likely a sample is mislabeled.
% While traditional methods treat the recommendation problem as a homoscedastic regression task~\cite{2007Probabilistic}, in this work, we reformulate it as a heterogeneous regression problem where samples have different variances.
In recommender systems, a large number of potential positive samples are often mistakenly labeled as 0. Training models on such data can result in a significant loss of useful information, leading to the development of poorly performing models. It is therefore crucial to quantify the likelihood of sample mislabeling. While traditional methods approach the recommendation problem as a homoscedastic regression task~\cite{2007Probabilistic}, in this work, we propose a reformulation of the problem as a heterogeneous regression task, where each sample has a different variance.

% We assume that the implicit feedback label $Y_{ui}$ follows the Gaussian Distribution $N(r_{ui},\sigma_{ui}^2)$, where $r_{ui}$ denotes the prediction of any recommendation model which is trained from the dataset $\mathcal{D}$.
% The variance $\sigma_{ui}^2$ represents the stability of the Gaussian Distribution, which is a variable learned from the implicit data. 
% A large variance $\sigma_{ui}^2$ usually indicates that the given label is unstable,\ie a label with large variance is likely to be incorrect.
% We thus use the variance of the label to quantify the likelihood of mislabeling, which is referred to as aleatoric uncertainty.
% Similar to \cite{2017What}, we define the variance $\sigma_{ui}^2$ as our aleatoric uncertainty of the label $Y_{ui}$. 
% \subsubsection{Uncertainty Estimator}\label{unestimator}
% We consider to model the uncertainty $\sigma_{ui}^2$ in a similar manner as the backbone model $r_{ui}=f_{\theta}(u,i)$.
% To ensure the non-negativity of $\sigma_{ui}^2$, we naturally consider to denote it by following the exponential form:
We assume that the implicit feedback label $Y_{ui}$ follows a Gaussian Distribution $N(r_{ui},\sigma_{ui}^2)$, where $r_{ui}$ represents the prediction of a recommendation model trained on the dataset $\mathcal{D}$. The variance $\sigma_{ui}^2$ represents the stability of the Gaussian Distribution and is a learned variable derived from the implicit data. A large value of $\sigma_{ui}^2$ indicates that the given label is unstable, meaning that a label with a large variance is likely to be incorrect. Therefore, we use the variance of the label to quantify the likelihood of mislabeling, which we refer to as aleatoric uncertainty. Similar to the approach in \cite{2017What}, we define the variance $\sigma_{ui}^2$ as our aleatoric uncertainty of the label $Y_{ui}$.
To model the uncertainty $\sigma_{ui}^2$, we follow a similar approach to the backbone model $r_{ui}=f_{\theta}(u,i)$. To ensure that $\sigma_{ui}^2$ is non-negative, we represent it in exponential form:
\begin{equation}\small
\sigma_{ui}^2=g_{\phi}(u,i)=\frac{e^{h_{\phi}(u, i)}}{K}.
\label{exponential}
\end{equation}
$K$ controls the scale of exponential function.
% Notice that the uncertainty of the label $Y_{ui}$ is a combination of the uncertainty signals from the user and item. 
% We learn latent item representation $q_i$ and user representation $p_u$, similar to recommender models, and combine them as $h_{\phi}(u, i)$. 
It should be noted that the uncertainty of the label $Y_{ui}$ is a result of a combination of uncertainty signals from both the user and the item. Therefore, we learn latent representations for items, denoted by $q_i$, and for users, denoted by $p_u$, as done in typical recommender models. We then combine these representations as $h_{\phi}(u, i)$ to determine the uncertainty associated with a given label.

As to item $i$, we learn a projection $f_{item}:e_i \rightarrow q_i$ to %mine the feature of item itself
mine the latent factors affecting uncertainty,
where $e_i$ denotes the one-hot encoding of item $i$.
For user representation, intuitively, users with similar item interactions should have similar uncertainty.
We employ the combination of all item representations in the user's historical interaction as the user representation. Formally, $p_u=\sigma(\frac{1}{\sqrt{|\mathcal{H}_u|}}\sum_{i\in \mathcal{H}_u}z_i),$
where $\mathcal{H}_u$ denotes the historical interaction set of user $u$, and $\sigma$
indicates an activation function. $z_i$ is the user history information encoded by another projection\footnote{This design is similar to \cite{koren2008factorization}, which validates the rationality of using two different projections.} $f_{user}:e_i \rightarrow z_i$.
Then $h_{\phi}(u, i)$ is simply defined as the inner product of item representation $q_i$ and user representation $p_u$, \ie $h_{\phi}(u,i)=<p_u,q_i>$. For briefness, we denote the value of $h_{\phi}(u, i)$ as {$s_{ui}$} in the rest of the paper. 
\subsection{Training Procedure}\label{sec:training}
A default choice for estimating the parameters of backbone model and uncertainty estimator is minimizing the negative log-likelihood of training samples. Formally, the negative log-likelihood of $Y_{ui}$ is $-logP(Y_{ui}|r_{ui},\sigma_{ui}^2)=\frac{(r_{ui}-Y_{ui})^2}{2\sigma_{ui}^2}+\frac{1}{2}log \ \sigma_{ui}^2$.
Due to the huge amount of training instances, we usually consider the mini-batch training strategy. 
We adopt the same user-batch strategy used in \cite{liang2018variational}. We first randomly sample a batch of users $\mathcal{U}_{batch}$ from $\mathcal{U}$, then the user batch loss $L(\mathcal{U}_{batch},\mathcal{D};\theta,\phi)$ can be formulated as:
\begin{equation}\small
\begin{split}
\sum_{u\in \mathcal{U}_{batch}, i \in \mathcal{I}}w_{ui}\left(
    \frac{(r_{ui}-Y_{ui})^2}{
        \frac{2}{K}e^{s_{u,i}}}+\frac{1}{2} \ s_{u,i}
\right)+\Omega,
\label{loss_overall}
\end{split}
\end{equation}
where $w_{ui}$ denotes the weight of different samples in the training set $\mathcal{D}$, and $\Omega$ denotes the regularization term.

Noticing that optimizing the two models simultaneously can lead to unstable issues and overfitting~\cite{yu2020sampler},
we propose to train them sequentially in an Expectation-Maximization like algorithm. In particular, we first train the backbone model as our expectation estimator without considering the uncertainty, and then train the uncertainty estimator while fixing the expectation model. 
Sequential training also simulates the situation where our method is grafted onto an existing model, which is required by industry applications. We also show the results of the joint learning of expectation and uncertainty in the experiments (\cf Table~\ref{variant}).
\subsubsection{Backbone Training}\label{expectation_training}
To alleviate the imbalance issue of positive and negative samples, we leverage a sampling strategy.
We assign the weight to each instance $w_{ui}$ as follows:
\begin{equation}\small
    w_{ui}\sim
   \begin{cases}
   1 &\mbox{$Y_{ui}=1$,}\\
   Bernoulli(\mu) &\mbox{$Y_{ui}=0$.}
   \end{cases}
   \label{weight}
\end{equation}
where $\mu$ denotes the sampling rate for negative samples.
The aleatoric uncertainty is not considered for the backbone model,  We set $s_{ui} = 0$ and use $l_2$-norm as regularization, $s_{ui}$ is thus fixed for all users and items. \ie $\Omega=\lambda||\theta||^2$, simplifying the training objective for backbone model as:
\begin{equation}\small
\begin{split}
&L(\mathcal{U}_{batch},\mathcal{D};\theta)=\sum_{u\in \mathcal{U}_{batch}, i \in \mathcal{I}}w_{ui}\left(
    \frac{(r_{ui}-Y_{ui})^2}{2}
\right)+\lambda ||\theta||^2.
\label{loss_backbone}
\end{split}
\end{equation}
The first term is essentially a mean square error, one of the common recommendation losses. 
The form of the loss is decided by the prior assumption of data distribution. Other losses like BPR \cite{2009BPR} corresponds to distributions other than Gaussian Distribution.
We belief Gaussian Distribution is a reasonable assumption since Equation ~\eqref{loss_backbone} can lead to stronger backbone models than BPR (\cf Figure~\ref{fair}).
\subsubsection{Uncertainty Estimator Training}
The uncertainty estimator is trained on top of the backbone model. In this stage, we also need to balance the positive and negative samples, although the learning objective is not the hard label of implicit data. 
To speed up training, we replace the sampling process by directly assigning fixed weight to each instance.
The weight $w_{ui}$ there can be formulated as:
\begin{equation}\small
    w_{ui}=
   \begin{cases}
   \alpha &\mbox{$Y_{ui}=1$,}\\
   1 &\mbox{$Y_{ui}=0$.}
   \end{cases}
   \label{weight}
\end{equation}
where $\alpha$ is a key hyperparameter for training the uncertainty estimator. More specifically, $\alpha$ can be adjusted to control the strength of 
emphasizing the tail items (\cf Figure~\ref{hyper}). 

To optimize the uncertainty estimator, we first derive the distribution of uncertainty $P(s_{ui}|r_{ui},Y_{ui})$. According to Bayes theorem, we can get:
\begin{equation}\small
    P(s_{ui}|r_{ui},Y_{ui})=\frac{P(Y_{ui}|r_{ui},s_{ui})P(r_{ui}|s_{ui})P(s_{ui})}{P(r_{ui},Y_{ui})}.
\end{equation}
Since the expectation and variance of a Gaussian Distribution are independent statistics~\cite{casella2021statistical}, $s_{ui}$ and $r_{ui}$ are independent. We have $P(r_{ui}|s_{ui})=P(r_{ui})$. Note that when training the uncertainty estimator, $r_{ui}$ is fixed and treated as a constant. Then we have $P(s_{ui}|r_{ui},Y_{ui}) \propto P(Y_{ui}|r_{ui},s_{ui})P(s_{ui})$. We assume that $s_{ui}$ has a prior of zero-mean Gaussian Distribution: $s_{ui} \sim N(0,\tau^2)$.
Combined with Equation \eqref{exponential}, we obtain the posterior probability of $s_{ui}$ and minimize its negative logarithm to optimize the parameters of uncertainty estimator. Formally,
\begin{equation}\small
    -logP(s_{ui}|r_{ui},Y_{ui})=\frac{(r_{ui}-Y_{ui})^2}{\frac{2}{K}e^{s_{ui}}}+\frac{1}{2}s_{ui}+\frac{s_{ui}^2}{\tau^2}+c,
\end{equation}
where $c$ denotes a constant. After simplifying the form, the final optimization objective is:
\begin{small}
\begin{equation}
\begin{split}
&L(\mathcal{U}_{batch},\mathcal{D};\phi)=\sum_{u \in \mathcal{U}_{batch},i \in \mathcal{I}}w_{ui}\left(
    \frac{(r_{ui}-Y_{ui})^2}{e^{s_{ui}}}+\beta s_{ui}+ \gamma s_{ui}^2
\right),
\label{loss}
\end{split}
\end{equation}
\end{small}
where $\beta$, $\gamma$ are hyperparameters.
This training process can be understood as finding the best variances such that the data likelihood is maximized.

After obtaining the optimal values of the variance, our model makes recommendations based on both of the expectation and aleatoric uncertainty.
$Pred_{ui}$ denotes the final prediction of the pair $(u,i)$. 
Given the pair $(u,i)$, the final prediction is $Pred_{ui}=(1-\lambda)r_{ui}+\lambda \sigma_{ui}$.
When $\lambda = 0 $, the prediction degenerates to the backbone model.

\begin{figure}[t]
	\centering
	%\subfigbottomskip=1pt
	\subfigure{
		\includegraphics[width=0.44\columnwidth]{pic/sigma_r_Yelp.png}
	}
	\subfigure{
		\includegraphics[width=0.44
		\columnwidth]{pic/sigma_r_Amazon.png}
	}
 	\vspace{-10pt}
	\caption{Relationship between $r_{ui}^2$ and $\sigma_{ui}^2$.}
	\vspace{-10pt}
\label{r_sigma}
\end{figure}


\subsection{Theoretical Analysis}\label{sec:algo}
In this subsection, we first show that the overall performance of the recommendation with aleatoric uncertainty is at least as good as the backbone models using expectation. The statement is further verified empirically with results from two real datasets (\cf Table~\ref{main result}). We then explain the mechanism of improving the tail performance.
%\subsubsection{Overall Performance}

\noindent \textbf{$\bullet$ Overall Performance. }
We first state the property that connects the aleatoric uncertainty with the expectation. 
\begin{theorem}
Denote the residual of the expectation as $\Delta_{ui}=r_{ui}-Y_{ui}$. 
For user $u$, denote the distributions of $\Delta_{ui}^2$ and $e^{s_{ui}}/K$ over the items as $p_u$ and $q_u$ respectively.
If the weights $w_{ui}$ are the same for all user-item pairs, the following inequality holds:
\begin{equation}\small
    L(\mathcal{D}) \ge \sum_{u}KL(p_{u}||q_{u}) + c,
\end{equation}
where $L(\mathcal{D})$ is the loss of uncertainty estimator in Equation \eqref{loss}; $KL(p_u||q_u)$ is the KL-Divergence of the two distributions; and $c$ is a constant. 
\end{theorem}
\wcx{
\textbf{Proof of Theorem 1}\label{proof}
The training objective of uncertainty estimator, \ie Equation (\ref{loss}) can be written as:
\begin{equation}
\small
\begin{split}
&L(D)=\sum_u\sum_{i}(\frac{\Delta_{ui}^2}{e^{s_{ui}}}+\beta s_{ui}+ \gamma s_{ui}^2)
\end{split}
\end{equation}
here we assume $w_{ui}$ or $\alpha$ in equation (\ref{weight}) is 1, but it is trivial to obtain a similar inequality for $\alpha \neq 1$.
We obtain the normalized distribution of $p_u$ and $q_u$ as where $K_{u}=\sum_{i}\Delta_{ui}^2, R_{u}=\sum_{i}e^{s_{ui}}$, and $p_{ui}$ and $q_{ui}$ denote the value of $p_u$ and $q_u$ on the $i$-$th$ item.
According to the common inequality: $lnx+1 \le x (x>0)$, we can derive the inequality:
\begin{equation}
\small
    \frac{\Delta_{ui}^2}{e^{s_{ui}}}=  \frac{\Delta_{ui}^2}{K_{u}}\frac{K_{u}}{e^{s_{ui}}}\ge \frac{\Delta_{ui}^2}{K_{u}}(ln\frac{\frac{\Delta_{ui}^2}{K_{u}}}{\frac{e_{s_{ui}}}{R_{u}}}+ln\frac{K_{u}^2}{R_{u}}+1-ln\Delta_{ui}^2)
\end{equation}
By substituting the above inequality into $L(D)$, we have:
\begin{equation}\small
\begin{split}
&L(\mathcal{D})\ge \sum_{u}\sum_{i}(p_{ui}(ln\frac{p_{ui}}{q_{ui}}-lnR_{u})+\beta s_{ui}+ \gamma s_{ui}^2)+c_1\\
&=\sum_{u}KL(p_{u}||q_{u})+\sum_{u}\sum_{i}(\beta s_{ui}+ \gamma s_{ui}^2 -lnR_{u})+c_1
\end{split}
\label{eq21}
\end{equation}
Assume that $s_{uk}=max_{i}s_{ui}$, we have $lnR_{u}\le ln|\mathcal{I}|e^{s_{uk}}=s_{uk}ln|\mathcal{I}|$ and $\mathcal{I}$ is the set of all items. According to the Extremum Theorem of a quadratic function, we can derive:
\begin{equation}
\begin{split}
&\beta s_{ui}+ \gamma s_{ui}^2 \ge \frac{-\beta ^2}{4\gamma} \ \ \ \ \ \ \  for \ i \neq k\\
&(\beta-ln|\mathcal{I}|) s_{uk}+\gamma s_{uk}^2 \ge \frac{-(\beta-ln|\mathcal{I}|) ^2}{4\gamma} \ for \ i = k
\end{split}
\end{equation}
Therefore, the second term in the RHS of the inequality (\ref{eq21}) is also lower bounded by a constant.
Overall, we can obtain the inequality:
\begin{equation}
\small
    L(\mathcal{D}) \ge \sum_{u}KL(p_{u}||q_{u})+c
\end{equation}
This completes the proof of the theorem.
}

The above theorem essentially states that the KL-Divergence between the distributions of expectation and uncertainty is bounded by the loss function that is being optimized. In other words, the lower the loss can be achieved, the closer the two distributions will become. Therefore, the expectation and the uncertainty are highly positively correlated, and thus the overall performance of uncertainty recommendation should be at least on par with the recommendation models using expectation. 

To further validate the above statement, we report the empirical results on two real world datasets in Figure \ref{r_sigma}. Specifically, we randomly select one user from each dataset and show the visual relationship between $r_{ui}^2$ and $\sigma_{ui}^2$. 
As shown in Figure \ref{r_sigma}, it is clear that expectation and uncertainty have strong linear positive correlation for both users, which confirms the theorem. The yellow line indicates the best fit line. Moreover, we calculate the mean pearson correlation coefficient on different datasets over the users, where it is 0.69 on Amazon-Book and 0.74 on Yelp (see dataset descriptions in Section \ref{ssec:exp_setting}).

\noindent \textbf{$\bullet$ Tail Performance. }
We also claim that using uncertainty to make recommendations improves the quality of tail items recommendations. 
The reason is that when a positive sample is not able to be retrieved by the expectation $r_{ui}$, its variance $\sigma_{ui}^2$ would be learned to be a large value. 
This positive sample is likely to be captured by our AUR model. Especially, when the hyperparameter $\alpha$ in Equation \eqref{weight} increases, the $\sigma_{ui}^2$ of tail items would also increase. Therefore, we name $\alpha$ as the \textbf{tail-controlling coefficient}.

We use an example to illustrate this statement in Table \ref{pop}. We select a user and four items from the Amazon-Book dataset to compare the learned expectations and uncertainties. The backbone model is MF. We count item popularity in the training set while the user feedback is retrieved from the testing set. From the table, we can see that $i_4$ has a much lower popularity compared to $i_1$, as well as its expectation.
Despite that item $i_1$ has been interacted many times, it is actually a true negative sample for the user.
Both the popularity and the expectation of $i_4$, a true positive sample, are the lowest among the four items, but it still has the highest uncertainty indicating that $i_4$ is a potential positive sample. We provide more analysis in the experiments.
\begin{table}
\small
\centering
\caption{Case study of selected user-item pairs. We show four items with their expectation, uncertainty, and popularity in Amazon to explain how AUR improves the tail performance. }
\vspace{-4mm}
\begin{tabular}{|c|cccc|}
\hline
Items         & $i_1$   & $i_2$   & $i_3$   & $i_4$   \\ \hline
Expectation   & 0.8038 & 0.7784 & 0.7654 & 0.4648 \\
Uncertainty   & 0.3188 & 0.2952 & 0.3050 & 0.3277 \\
Popularity    & 128    & 44     & 59     & 40     \\
User Feedback & 0      & 0      & 0      & 1      \\ \hline
\end{tabular}
\label{pop}
\vspace{-6mm}
\end{table}

\subsection{Discussion}\label{sec:discussion}
\noindent \textbf{$\bullet$ Relevance to Sample Weighting. }
We first discuss the connections and distinctions between our approach and previous methods. 
In the previous discussion, \cite{2009Collaborative,reweight1} heuristically assigned weights $c_{ui}$ to each training sample. In our work, if we fix $s_{ui}=log(\frac{1}{c_{ui}})$ and $\alpha=1$ in Equation \eqref{loss} to optimize the backbone model, our approach is equivalent to \cite{2009Collaborative,reweight1}.
Intuitively, for the positive samples, high correlation between $(u,i)$ indicates low variance \cite{2009Collaborative}. For the negative samples, high correlation indicates that the item $i$ might be a potential positive sample for user $u$, resulting in a high variance \cite{reweight1}.
Therefore, assigning fixed weights to re-weight MSE loss in the training process is essentially to determine the uncertainty of each sample.
Previous methods specify/fix the variance to learn the expectation. In contrast, our approach first learns an expectation, and then estimates the variance based on the learned expectation. During the recommendation stage, previous methods recommend items using expectation while we make recommendations with variance to better capture the uncertainty in the data.
\noindent \textbf{$\bullet$ Relevance to Probabilistic Methods. }
Similar to AUR, some probabilistic models, \textit{e.g.}, PMF \cite{2007Probabilistic} and ExpoMF \cite{2016Modeling}, also assume the implicit labels obey Gaussian Distributions. Differently, they take the variances of Gaussian Distributions as hyper-parameters, and assume all $(u,i)$ pairs have the same variances. 
AUR estimates the variances for each $(u,i)$ pair with the proposed learning strategy, obtaining more accurate uncertainties at a fine-grained user-item pair level.
Moreover, these probabilistic models generate recommendations with the predicted expectations, which may over-recommend popular items,as discussed in Section~\ref{exp_prob}. Fundamentally different to them, AUR makes recommendations based on the uncertainties, aiming at providing more accurate and more balanced recommendations.
